From Literature to Hypotheses: An AI Co-Scientist System for Biomarker-Guided Drug Combination Hypothesis Generation

The rapid growth of biomedical evidence makes it difficult to translate biomarker mechanisms into actionable drug combination hypotheses. We present CoDHy, an interactive AI co-scientist for biomarker-guided hypothesis generation in oncology. CoDHy constructs task-specific knowledge graphs from curated databases and biomedical literature, then combines graph embeddings with agent-based reasoning to generate, validate, and rank evidence-grounded drug combinations. Through a web interface, researchers specify the biomarker, cancer context, and literature scope; inspect supporting evidence and intermediate results; and iteratively refine the generated hypotheses. The demonstration presents CoDHy's end-to-end workflow and shows how researchers can interactively explore and compare mechanistically supported drug combinations while remaining in control of hypothesis prioritization.

==> sections/Evaluation.tex <==
\section{Evaluation Results and Analysis}
We evaluate CoDHy through a small set of controlled case studies and comparative experiments designed to assess (i) interpretability, (ii) evidence grounding, and (iii) the contribution of key architectural components. All experiments follow a fixed experimental protocol to ensure comparability across system variants.

\subsection{Experimental Setup}

\paragraph{Scenarios.}
We define a fixed set of seven evaluation scenarios, each specified by a (biomarker, cancer type) pair (e.g., \textbf{(EGFR, Lung Squamous Cell Carcinoma)}). This scenario list is frozen prior to experimentation and reused across all methods. The full list is provided in \red{Table~\ref{tab2:eval_scenario} (Appendix)}.

\paragraph{Global settings.}
Unless stated otherwise, all experiments retrieve \textbf{N = 50} PubMed abstracts and generate \textbf{H = 4} hypotheses per scenario. We use the same language model, \textbf{Llama 3.1}\footnote{\url{https://huggingface.co/meta-llama/Llama-3.1-8B-Instruct}} \red{via the Hugging Face inference provider}, with identical model parameters across all methods.

\paragraph{Methods compared.}
We evaluate three variants:
\textbf{Full CoDHy}: complete system with knowledge graph construction, RotatE-based inference, \SB{rule-based path consistency filtering, feedback-driven revision, taboo-list-guided regeneration}, and validation agents; \textbf{LLM-only}: direct prompting baseline without knowledge graph or graph embeddings; and \textbf{No-Embedding}\footnote{Referred to as \texttt{No-Node2Vec} in the codebase, retained from the earlier Node2Vec-based implementation; the ablation now removes RotatE-based inference specifically.}: ablated variant using direct knowledge graph evidence only, without embedding-based inference.

For each generated hypothesis, we log structured outputs including rank, composite scores, validation verdicts, novelty status, and supporting PubMed identifiers.

\subsection{End-to-End Case Study}
We demonstrate CoDHy on the scenario 
\textbf{(Breast Invasive Carcinoma, EGFR)}.
The system retrieves 50 PubMed abstracts, constructs a task-specific
knowledge graph, and generates four ranked hypotheses:

\noindent\rule{\columnwidth}{0.4pt}

\textbf{H1 (Score=9.0, Verdict: Proceed)}  
\textit{Afatinib + Palbociclib}  
Mechanism: Resistance reversal via EGFR inhibition and CDK4/6 blockade.  
Rationale: Direct graph evidence.  
Evidence: PMIDs 41723568, 41723552, 41723543.

\medskip

\textbf{H2 (Score=9.0, Verdict: Caution)}  
\textit{Lapatinib + AZD9291}  
Mechanism: Synthetic lethality through dual EGFR pathway targeting.  
Rationale: Inferred embedding similarity.  
Evidence: PMIDs 32547705, 29103264.

\medskip

\textbf{H3 (Score=9.0, Verdict: Proceed)}  
\textit{Osimertinib + Fulvestrant}  
Mechanism: Estrogen-dependent synthetic lethality.  
Rationale: Inferred similarity.  
Evidence: PMIDs 41723568, 41723543.

\medskip

\textbf{H4 (Score=9.0, Verdict: Proceed)}  
\textit{Ceritinib + Everolimus}  
Mechanism: Resistance reversal via mTOR pathway inhibition.  
Rationale: Direct graph evidence.  
Evidence: PMIDs 41706704, 41622283.

\noindent\rule{\columnwidth}{0.4pt}

This example illustrates three CoDHy properties: (1) generation of multiple mechanistically diverse hypotheses, (2) distinction between graph-supported and embedding-inferred candidates, and (3) explicit attachment of literature evidence and validation verdicts.
Full structured outputs are provided in  \red{Appendix~\ref{sec:appendix_outputs}}.

\subsection{Comparative Evaluation}
We next assess the contribution of structured evidence integration and embedding-based inference.

\paragraph{Metrics.}
Across all scenarios and system variants, we compute the following metrics: (i) \textbf{Novelty rate} (exact and context-aware), (ii) \textbf{Evidence coverage}, (iii) \textbf{Proceed@1 / Proceed@3}, and (iv) \textbf{Diversity}. Formal metric definitions are provided in \red{Appendix~\ref{sec:metric-definitions}}.

\paragraph{Results.}
\input{images/comparitive_evaluation}
%illustrates the trade-off between literature retrieval and discovery in hypothesis generation by comparing 
Table~\ref{tab3:main_comparison} compares the full CoDHy system, LLM-only baseline, and No-Node2Vec variant across multiple criteria. The LLM-only baseline achieves the highest evidence coverage (0.93) and Proceed@1 rate (0.71), reflecting its tendency to generate well-documented literature-supported combinations. However, it exhibits substantially lower exact novelty (10.71\%), suggesting a retrieval-oriented bias. Removing embedding-based inference (No-Node2Vec) increases exact novelty (28.57\%) while maintaining strong evidence grounding (0.72), indicating that direct knowledge graph connections can partially mitigate retrieval bias. The full CoDHy system achieves the highest exact novelty (35.71\%), while maintaining high combination diversity (0.89) and competitive evidence coverage. Overall, these results suggest that integrating structured knowledge graphs with embedding-based inference enables a better balance between novelty, evidence support, and hypothesis diversity than either component alone.

\subsection{Ranking Quality}
We evaluate whether CoDHy's composite scoring function ranks higher-quality hypotheses using standard information retrieval metrics.

\paragraph{Metrics.}
We report nDCG@3 and Mean Reciprocal Rank (MRR). Formal definitions of both metrics and their implementation in our setting are provided in \red{Appendix~\ref{sec:metric-definitions}.}

\paragraph{Results.}
To report MRR and nDCG@3 for our experiment, we use relevance label (\emph{Literature Supported} = 1, \emph{Novel/Unsupported} = 0) for the combinations. Table~\ref{tab4:ranking} shows that the LLM-Only baseline achieves near-perfect retrieval metrics (MRR: 0.93), reflecting its tendency to memorize existing standard-of-care combinations. In contrast, Full CoDHy achieves a lower MRR (0.74), a direct consequence of its deliberate design objective: rather than already-published combinations, CoDHy promotes biologically plausible but previously unpublished (novel) combinations through embedding-based inference. The reduction in the retrieval-oriented ranking metric (MRR), therefore, indicates a successful transition from a search-retrieval paradigm toward a discovery-oriented paradigm.
\input{images/Ranking_quality}

\subsection{LLM-as-Judge Evaluation}
\SB{To assess CoDHy against general-purpose and biomedical-domain LLMs directly, rather than only against its own ablations, we additionally compare full CoDHy to five zero-shot baseline models using an independent, blind LLM-as-Judge protocol.}

\paragraph{Zero-shot baselines.}
\SB{For the same (biomarker, cancer type, hypothesis count) inputs used by CoDHy, each of five LLMs is separately prompted to propose drug-combination hypotheses using only its own pretrained knowledge, with no knowledge graph, embeddings, consistency filtering, or taboo/feedback context. This isolates the contribution of CoDHy's structured pipeline from the contribution of the underlying LLM's own biomedical knowledge.}

\paragraph{Judge panel and rubric.}
\SB{Five LLMs judge every hypothesis (from CoDHy and from the baselines) on a fixed, blind rubric: DeepSeek-R1\footnote{\url{https://huggingface.co/deepseek-ai/DeepSeek-R1}} and Qwen3-235B-A22B-Instruct-2507\footnote{\url{https://huggingface.co/Qwen/Qwen3-235B-A22B-Instruct-2507}} as general-purpose, frontier-class judges from different labs and architectures; and JSL-MedLlama-3-8B-v2.0\footnote{\url{https://huggingface.co/johnsnowlabs/JSL-MedLlama-3-8B-v2.0}}, Llama3-OpenBioLLM-8B\footnote{\url{https://huggingface.co/aaditya/Llama3-OpenBioLLM-8B}}, and BioMistral-7B-SLERP\footnote{\url{https://huggingface.co/BioMistral/BioMistral-7B-SLERP}} as biomedical-domain fine-tunes spanning two base architectures (Llama-3 and Mistral). Llama-3.1-8B-Instruct, the model used for CoDHy's own generation and validation, is deliberately excluded from the judge panel to avoid self-preference bias. Each hypothesis is shown to a judge with no indication of which system produced it (\emph{combination}, \emph{mechanism}, \emph{reasoning}, and \emph{supporting evidence} fields only), and scored on an integer 1--5 scale across seven dimensions: novelty, biological plausibility, evidence grounding, mechanistic explanation, specificity, testability, and clinical relevance. Whenever a baseline hypothesis would be judged by the same model that generated it, that judge is excluded for that item to prevent a model from scoring its own output. Each (hypothesis, judge) pair is scored 3 times to support test-retest reliability reporting.}

\paragraph{Inter-judge and test-retest reliability.}
\SB{We report Krippendorff's alpha and ICC(C,k)/ICC(A,k) per scoring dimension as measures of inter-judge agreement, per-judge mean/std as a bias check, pairwise Spearman correlation between judges, repeat-consistency (agreement of the same judge with itself across the 3 repeats) as a test-retest reliability check, and the correlation between the Validation Agent's own in-pipeline plausibility score and the external judge panel's mean score, as a sanity check on self-validation. Table~\ref{tab5:llm_judge_agreement} reports these statistics.}
\input{images/llm_judge_agreement}

\paragraph{Pairwise comparison.}
\SB{For each baseline, a blind pairwise A/B comparison is run against CoDHy on matched (biomarker, cancer type) items, with position (A vs.\ B) randomized per call to control for position bias and the winning side attributed back to the underlying system regardless of shown position. Table~\ref{tab6:pairwise} reports win/tie/loss percentages.}
\input{images/pairwise_comparison}

\paragraph{Objective metrics.}
\SB{Table~\ref{tab7:objective_metrics} reports Evidence Coverage, (exact) Novel Combination Rate, Diversity, Citation Precision, and wall-clock Runtime per system. Evidence Coverage, Novel Combination Rate, and Citation Precision require the PubMed-grounded validation step CoDHy's own hypotheses go through; zero-shot baselines skip validation by design and are therefore reported as not applicable for those three columns, rather than as zero.}
\input{images/objective_metrics}

%\subsection{Novelty Assessment}
%We assess novelty using two complementary criteria. A hypothesis is considered \emph{novel-exact} if no PubMed results are returned for the query ``DrugA AND DrugB'', and \emph{novel-in-context} if no results are returned for ``DrugA AND DrugB AND CancerType''. Both hit counts are logged and reported.

%\paragraph{Results.}
%\input{images/Novelty_assessment}
%Table~\ref{tab5:novelty} shows that the full CoDHy system achieves consistently higher novelty under both exact and context-aware criteria than ablated and LLM-only variants. While the LLM-only baseline generates superficially novel combinations, many lack contextual relevance, whereas integrating structured knowledge and embedding-based inference supports context-aware novelty.

==> table/judge_deepseek_only.tex <==
\begin{table}[t]
\centering
\caption{Scores from DeepSeek-R1 alone, the panel's only judge with no generation stake. Bold marks the highest score per criterion.}
\label{tab:deepseek-only}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
System & Novelty & Bio. Plausibility & Evidence Grounding & Mechanistic Clarity & Specificity & Testability \\
\midrule
CoDHy              & 3.1 & \textbf{3.7} & \textbf{2.8} & 2.6 & \textbf{3.3} & \textbf{3.3} \\
MedGemma-1.5-4B    & \textbf{3.3} & 2.9 & 2.7 & 2.5 & 3.2 & 3.0 \\
Qwen3-8B           & 2.7 & 2.7 & 1.7 & 2.7 & 2.8 & 3.0 \\
JSL-MedLlama-3-8B  & 2.5 & \textbf{3.7} & 2.6 & \textbf{3.1} & 3.2 & 3.1 \\
OpenBioLLM-8B      & 2.6 & 3.2 & 1.5 & 2.5 & 2.7 & 3.1 \\
BioMistral-7B      & 2.8 & 3.0 & 2.3 & 2.9 & 3.2 & 3.0 \\
\bottomrule
\end{tabular}}
\end{table}

==> table/judge_matched_n.tex <==
\begin{table}[t]
\centering
\caption{Judge-count-matched comparison. For each baseline, CoDHy's score is recomputed using only the five judges that exclude that baseline's own model, matching the baseline's self-excluded $n=5$. Cells show CoDHy (matched) / Baseline, with the winning value in bold.}
\label{tab:matched-n}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
Baseline excluded & Novelty & Bio. Plausibility & Evidence Grounding & Mechanistic Clarity & Specificity & Testability \\
\midrule
MedGemma-1.5-4B   & 2.9/\textbf{3.3} & \textbf{4.0}/2.9 & \textbf{3.2}/2.4 & \textbf{3.3}/2.9 & \textbf{3.70}/3.20 & \textbf{3.64}/3.20 \\
Qwen3-8B          & 2.9/\textbf{3.0} & \textbf{4.1}/3.2 & \textbf{3.5}/2.2 & \textbf{3.2}/3.1 & \textbf{3.82}/3.28 & \textbf{3.54}/3.08 \\
JSL-MedLlama-3-8B & \textbf{2.9}/2.8 & \textbf{4.0}/3.8 & \textbf{3.3}/3.0 & 3.2/\textbf{3.3} & \textbf{3.66}/3.36 & \textbf{3.50}/3.28 \\
OpenBioLLM-8B     & \textbf{2.9}/\textbf{2.9} & \textbf{4.0}/3.3 & \textbf{3.2}/1.9 & \textbf{3.3}/2.8 & \textbf{3.64}/2.90 & \textbf{3.58}/2.90 \\
BioMistral-7B     & \textbf{2.9}/2.7 & \textbf{4.0}/3.1 & \textbf{3.2}/2.2 & \textbf{3.4}/3.0 & \textbf{3.84}/3.14 & \textbf{3.54}/3.04 \\
\bottomrule
\end{tabular}}
\end{table}
